Unpacking Robustness in Inflectional Languages: Adversarial Evaluation and Mechanistic Insights

Various techniques are used in the generation of adversarial examples, including methods such as TextBugger which introduce minor, hardly visible perturbations to words leading to changes in model behaviour. Another class of techniques involves substituting words with their synonyms in a way that preserves the text's meaning but alters its predicted class, with TextFooler being a prominent example of such attacks. Most adversarial example generation methods are developed and evaluated primarily on non-inflectional languages, typically English. In this work, we evaluate and explain how adversarial attacks perform in inflectional languages. To explain the impact of inflection on model behaviour and its robustness under attack, we designed a novel protocol inspired by mechanistic interpretability, based on Edge Attribution Patching (EAP) method. The proposed evaluation protocol relies on parallel task-specific corpora that include both inflected and syncretic variants of texts in two languages -- Polish and English. To analyse the models and explain the relationship between inflection and adversarial robustness, we create a new benchmark based on task-oriented dataset MultiEmo, enabling the identification of mechanistic inflection-related elements of circuits within the model and analyse their behaviour under attack.

==> sections/explainability.tex <==
\section{Edge Attribution Patching}
In recently growing field of \textbf{Mechanical Interpretability (MI)} researchers aim to explain the behaviour of the model by measuring changes inside the model. One of the techniques used in MI is circuit discovery. Identifying circuits in language models can be expensive due to the challenge of pinpointing essential components and the main connections linking them. In order to effectively obtain circuits \citep{nanda2023} developed \textbf{Edge Attribution Patching (EAP)}, a technique that estimates the impact of connections with minimal computational passes through the model. The \textbf{Edge Attribution Patching with Integrated Gradients (EAP-IG)} \cite{hanna2024have} is an improvement over the EAP method which includes the integrated gradient technique (IG) \cite{DBLP:conf/icml/SundararajanTY17} into the circuit recognition. The integrated gradients addition aims to improve the EAP method when facing zero gradients regions between clean and corrupted response.

% , which is finding minimal subgraph of model components like attention heads and MLPs.==

% \paragraph{Edge Attribution Patching (EAP)}

% To address the efficiency issue, \citep{nanda2023} developed edge attribution patching (EAP), a method that estimates the impact of connections with minimal computational passes through the model. The effectiveness of EAP is supported by its high overlap with manually found circuits, a common measure of success in circuit-finding research. EAP is based on a gradient computation procedure
% that is used to approximate causal interventions on each model's edge with two forward passes and one backward pass.
% The EAP describes the transformer model as a computational graph, where the circuit executing a specific task can be represented as a subset of nodes and edges of the original graph. 
% % In this concept input for node $v$ can be expressed using the following formula:
% % $\sum_{e\in E_v} i_e \cdot z_u + (1 - i_e) \cdot z'_u$  where $v$ is a node in model, $E_v$ is a set of edged directed to node $v$, $i_e$ is a binary valued that indicated if edge $e$ is in the circuit, $z_u$ is output of node $u$ for clean run and $z'_u$ is the output for corrupted run.
% In order to find the circuit, the scoring function for each model edge is needed. The EAP proposes an approximate value by using the negative loss change in each edge between clean and corrupted runs. 

% % in loss $L$ caused by corrupting $e=(u, v)$. %, with formula:  

% % $$(z'_u - z_u)^T \nabla_vL(s)$$

% % where $\nabla_vL(s)$ is  gradient change in loss $L$ for input of node $v$. Loss change can be converted into score metric $M$, by taking $L(s) = - M(s)$. The loss change is computed for forward one pass for clean and corrupted inputs, and backward pass on clean input.
% % todo PW: tu można jakoś spróbować półformalnie zapisać metodę wzorując się na fragmentach artykułu o EAP-IG
 


% % The EAP-IG score function for edge $e$ can be described as:
% % $$(z'_u - z_u)\frac{1}{m}\sum_{k=1}^{m}\frac{\partial L(z' + \frac{k}{m}(z - z'))}{\partial z_v}$$ where $m$ is the number of integral approximation steps, $z$ is token embeddings for clean input and $z'$ is token embedding for corrupted input. 
% The score function uses accumulation of gradient, which helps in situation of facing zero gradients along path between clean and corrupted activations.

==> tables/attack_test_dataset.tex <==
\begin{table}
    \caption{Attack Success Rate (ASR) with respect to adversarial attack methods. Numerical values are shown as percentages, indicating the proportion of samples with adversarial examples out of the total number of examples.}
    \label{table:test_attack_succ}
    \centering
    \begin{tabular}{|l|l|r|r|r|r|r|}
    \hline
    Dataset & Lang. & TF [\%] & TB [\%] & WNTF [\%] & BA [\%] \\
    \hline
    AG\_News & ENG & 6.35 & \textbf{12.64} & 7.31 & 6.22 \\ \hline
    IMDB & ENG & 15.07 & \textbf{24.52} & 14.05 & 8.41\\ \hline
    Wiki\_PL & PL & 8.93 & \textbf{13.66} & 8.93 & 6.40 \\ \hline
    MultiEmo & PL & 8.97 & \textbf{11.32} & 5.88 & 4.41 \\ \hline
    CSFD & CZ & 14.80 & \textbf{33.58} & 5.70 & 6.91 \\ \hline
    CTDC & CZ & 20.14 & \textbf{27.13} & 5.65 & 17.21 \\
    \hline
    \end{tabular}
\end{table}


==> tables/detection_bert.tex <==
\begin{table}[htb]
    \caption{Attack detection results for BERT-based models.}
    \label{table:detect_eval_cls}
    \centering
    \begin{tabular}{|l|r|r|r|}
    \hline
    Language & Accuracy [\%] & F1 [\%] & ROC\_AUC [\%] \\ \hline
    English & 77.40 & 77.34 & 91.26 \\ \hline
    Polish & 65.72 & 64.73 & 80.13 \\ \hline
    Czech & \textbf{87.77} & \textbf{85.45} & \textbf{95.03} \\ \hline
    Multilingual & 80.71 & 80.09 & 91.49 \\ \hline
    \end{tabular}
\end{table}

==> tables/detection_cls_all.tex <==
\begin{table}[htb]
    \caption{Wykryte ataki na modele z podziałem na zbiory danych, dla modelu wielojęzycznego (LaBSE). Wartości numeryczne zostały wyrażone w procentach jako dokładność predykcji dla każdej z dwóch klas.}
    \label{table:detect_prc_all}
    \centering
    \begin{tabular}{|l|l|r|r|}
    \hline
    Dataset & Lang. & Class ''0'' (Org) [\%] & Class ''1'' (Attack) [\%] \\ \hline
    AG\_News & ENG & \textbf{99.35} & 65.90 \\ \hline
    IMDB & ENG &\textbf{88.41}& 81.50 \\ \hline
    Wiki\_PL & PL & \textbf{99.14} & 63.48  \\ \hline
    Multi\_Emo & PL & \textbf{96.61} & 53.58 \\ \hline
    CSFD & CZ & \textbf{94.86} & 78.53  \\ \hline
    CTDC & CZ & \textbf{99.11} & 66.71 \\ \hline
    \end{tabular}
\end{table}

==> tables/detection_cls_bert.tex <==
\begin{table}[htb]
    \caption{Detected attacks on models by dataset, for BERT-based models for each language. Numerical values are expressed as percentages, representing prediction accuracy for each of the two classes.}
    \label{table:detect_prc_lang}
    \centering
    \begin{tabular}{|l|l|r|r|r|r|}
    \hline
    \multirow{2}{*}{Dataset} & \multirow{2}{*}{Lang.} & \multicolumn{2}{|c|}{Class ''0'' (Org) [\%]} & \multicolumn{2}{|c|}{Class ''1'' (Attack) [\%]}\\
    && BERT & LaBSE & BERT & LaBSE \\ \hline
    AG\_News & ENG & \textbf{99.77} & 99.35 & 57.80 & 65.90\\ \hline
    IMDB & ENG & \textbf{98.33} & 88.41 & 67.26 & 81.50\\ \hline
    Wiki\_PL & PL & 99.09 & \textbf{99.14} & 45.26 & 63.48 \\ \hline
    Multi\_Emo & PL & \textbf{98.82} & 96.61 & 29.20 & 53.58 \\ \hline
    CSFD & CZ & 91.33 & \textbf{94.86} & 84.85 & 78.53\\ \hline
    CTDC & CZ & 93.01 & \textbf{99.11} & 90.15 & 66.71  \\ \hline
    \end{tabular}
\end{table}


    % AG\_News & ENG & \textbf{99.35} & 65.90 \\ \hline
    % IMDB & ENG &\textbf{88.41}& 81.50 \\ \hline
    % Wiki\_PL & PL & \textbf{99.14} & 63.48  \\ \hline
    % Multi\_Emo & PL & \textbf{96.61} & 53.58 \\ \hline
    % CSFD & CZ & \textbf{94.86} & 78.53  \\ \hline
    % CTDC & CZ & \textbf{99.11} & 66.71 \\ \hline

==> tables/detection_ds.tex <==
\begin{table}
    \caption{Attack detection train data. The datasets consist of two parts: unmodified (original) examples and modified examples generated to create adversarial examples. The datasets were divided into mutually exclusive training and test subsets.}
    \label{table:detect_dataset}
    \centering
    \begin{tabular}{|l|r|r|r|r|}
    \hline
    Language & Original & Attacked & Train & Test \\ \hline
    English & 2 592 & 5 600 & 6 553 & 1 639 \\ \hline
    Polish & 1 090 & 1 664 & 2 203 & 551 \\ \hline
    Czech & 3 143 & 12 237 & 12 304 & 3 076 \\ \hline
    Multilingual & 6 825 & 19 501 & 21 060 & 5 266 \\
    \bottomrule
    \end{tabular}
\end{table}
